GrAFT-PDX: Growth and Failure-Time Modeling of Patient-Derived Xenograft Experiments

Cancer drugs are often evaluated for efficacy in mice before proceeding to human clinical trials. To do this, human tumors are engrafted onto immune-incompetent mice to create a patient-derived xenograft (PDX). Engrafted tumors can be propagated to evaluate multiple drugs, but the time and costs involved in PDX studies limit high throughput drug screens in mice. Here we present GrAFT-PDX, a Bayesian model of PDX drug screens that aims to reduce the PDX screening burden by enabling imputation of missing experiments and early stopping of likely unsuccessful drugs. Unlike conventional survival or growth models, GrAFT-PDX jointly predicts tumor growth and survival outcomes using a learned latent function decomposition. In experiments on a large-scale PDX dataset, GrAFT-PDX outperforms Cox proportional hazards models at predicting time of death, outperforms machine learning baselines at predicting tumor growth, and recovers known gene-treatment relationships without genomic input.

==> preamble_aoas.tex <==
% AOAS-specific package choices.

\RequirePackage{amsmath,amssymb,amsthm}
\RequirePackage{mathtools}

\usepackage{relsize}

% Only load hyperref if AOAS accepts it for your use case.
% \RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}

% Since body uses \Cref and common preamble loads cleveref,
% keep theorem naming minimal here unless needed.

\startlocaldefs
\endlocaldefs
